FireFly A Synthetic Dataset for Ember Detection in Wildfire

This paper presents "FireFly", a synthetic dataset for ember detection created using Unreal Engine 4 (UE4), designed to overcome the current lack of ember-specific training resources. To create the dataset, we present a tool that allows the automated generation of the synthetic labeled dataset with adjustable parameters, enabling data diversity from various environmental conditions, making the dataset both diverse and customizable based on user requirements. We generated a total of 19,273 frames that have been used to evaluate FireFly on four popular object detection models. Further to minimize human intervention, we leveraged a trained model to create a semi-automatic labeling process for real-life ember frames. Moreover, we demonstrated an up to 8.57% improvement in mean Average Precision (mAP) in real-world wildfire scenarios compared to models trained exclusively on a small real dataset.

==> Conclusion.tex <==
\section{Conclusions} 
We designed a tool to automatically generate synthetic labeled dataset with dense small targets, and made the parameters controlling the diversity of the dataset adjustable based on UE. Using this approach, combined with reconstructions of forest scenes and simulations of ember trajectories, we released the large-scale synthetic dataset FireFly for ember detection. Our dataset consists of 19,273 images with high diversity. We tested the dataset on popular object detection models and demonstrates the relative effectiveness of YOLOv7. Using our training strategies for the real wildfire scene, the optimal mAP reaches 0.756 at $IoU=0.5$, and 0.277 at $IoU=0.5:0.95$, which is 7.5\% higher than training solely on a small semi-automatically-labelled real dataset. In addition, our training strategy achieves higher accuracy with fewer epochs than training only with the real dataset. These results suggest our tool and dataset provide an effective framework for ML-based detection of real-life wildfire embers.
%Combining all these, we provide an implementable solution to ember detection in real wildfire scenarios.
